Instance-dependent uniform tail bounds for empirical processes

We formulate a uniform tail bound for empirical processes indexed by a class of functions, in terms of the individual deviations of the functions rather than the worst-case deviation in the considered class. The tail bound is established by introducing an initial ``deflation'' step to the standard generic chaining argument. The resulting tail bound is the sum of the complexity of the ``deflated function class'' in terms of a generalization of Talagrand's $\gamma$ functional, and the deviation of the function instance, both of which are formulated based on the natural seminorm induced by the corresponding Cram\'{e}r functions. Leveraging another less demanding natural seminorm, we also show similar bounds, though with implicit dependence on the sample size, in the more general case where finite exponential moments cannot be assumed. We also provide approximations of the tail bounds in terms of the more prevalent Orlicz norms or their ``incomplete'' versions under suitable moment conditions.

==> preamble.tex <==
% \PassOptionsToPackage{natbib=true}{biblatex}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{amsmath, amsthm}
\usepackage{enumitem}

\makeatletter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Textclass specific LaTeX commands.
\theoremstyle{plain}
\newtheorem{thm}{\protect\theoremname}
\newtheorem{cor}{\protect\corollaryname}
\newtheorem{lem}{\protect\lemmaname}
\newtheorem{prop}{\protect\propositionname}
\theoremstyle{definition}
\newtheorem{defn}{\protect\definitionname}
\newtheorem{exmp}{\protect\examplename}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.


\usepackage[serif]{macros4tex}
\usepackage[unicode=true,pdfusetitle,
	bookmarks=true,bookmarksnumbered=false,bookmarksopen=false,
	breaklinks=false,pdfborder={0 0 0},pdfborderstyle={},backref=false,colorlinks=true]
{hyperref}
\hypersetup{
	urlcolor = URLColor,
	citecolor = CiteColor,
	linkcolor = LinkColor}

\usepackage[capitalise, noabbrev, nameinlink]{cleveref}
\crefname{thm}{Theorem}{Theorems}
\crefname{lem}{Lemma}{Lemmas}
\crefname{cor}{Corollary}{Corollary}
\crefname{prop}{Proposition}{Propositions}
\crefname{defn}{Definition}{Definitions}
\crefname{exmp}{Example}{Examples}
\crefname{problem}{Problem}{Problems}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefformat{equation}{#2#1#3}


\AtBeginDocument{
	%\DeclareFieldFormat{labelalpha}{\thefield{entrykey}}
	%\DeclareFieldFormat{extraalpha}{}
	\DeclareFieldFormat{titlecase:title}{\MakeSentenceCase*{#1}}
	\DeclareFieldFormat{titlecase:maintitle}{#1}
	\renewbibmacro{in:}{}
	\ifdefined\volnumdelim
		\renewcommand*{\volnumdelim}{\addcolon\space}
	\fi
	\renewcommand*{\ref}[1]{\cref{#1}}
}

% \usepackage{geometry}
% \geometry{verbose,tmargin=1in,bmargin=1in,lmargin=1in,rmargin=1in}

% \usepackage{refcheck}
% \newcommand{\refcheckize}[1]{%
%   \expandafter\let\csname @@\string#1\endcsname#1%
%   \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
%     \csname @@\string#1\endcsname{##1}\wrtusdrf{##1}}%
%   \expandafter\let\expandafter#1\csname relax\string#1\endcsname
% }
% \refcheckize{\cref}
% \refcheckize{\Cref}
\makeatother
%%%

%%% Now we add the reference commands we want refcheck to be aware of
% \refcheckize{\cref}
% \refcheckize{\Cref}

\usepackage[english]{babel}
\usepackage{csquotes}

\ifcsname bibltxstyle\endcsname
\else
	\newcommand{\bibltxstyle}{{ext-alphabetic}}
\fi
\usepackage[%
style=\bibltxstyle,
% style=ext-numeric, 
backend=biber, natbib=true, backref=true, giveninits=true, useprefix = true, sorting=nyt, url=false, isbn=false, eprint=true, doi=false, maxalphanames=4, minalphanames=4, minbibnames=6, maxbibnames=99]{biblatex}

\AtEveryBibitem{
	\ifentrytype{book}{}{% Remove publisher and editor except for books
		\clearlist{publisher}
		\clearname{editor}
	}
}
\DeclareFieldFormat{titlecase:title}{\MakeSentenceCase*{#1}}
% \DeclareFieldFormat{titlecase:maintitle}{#1}
\renewbibmacro{in:}{}

\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\corollaryname}{Corollary}
\providecommand{\theoremname}{Theorem}
\providecommand{\definitionname}{Definition}
\providecommand{\examplename}{Example}
